Probabilistic Bounds on the End-to-End Delay of Service Function Chains using Deep MDN

Ensuring the conformance of a service system's end-to-end delay to service level agreement (SLA) constraints is a challenging task that requires statistical measures beyond the average delay. In this paper, we study the real-time prediction of the end-to-end delay distribution in systems with composite services such as service function chains. In order to have a general framework, we use queueing theory to model service systems, while also adopting a statistical learning approach to avoid the limitations of queueing-theoretic methods such as stationarity assumptions or other approximations that are often used to make the analysis mathematically tractable. Specifically, we use deep mixture density networks (MDN) to predict the end-to-end distribution of the delay given the network's state. As a result, our method is sufficiently general to be applied in different contexts and applications. Our evaluations show a good match between the learned distributions and the simulations, which suggest that the proposed method is a good candidate for providing probabilistic bounds on the end-to-end delay of more complex systems where simulations or theoretical methods are not applicable.

==> normal_approx.tex <==
\section{Evaluation of an Emergency Room Model}\label{eval}

%\begin{figure*}[t!]
%\centering
%\includegraphics[scale=0.38]{onoff_scatter.png}
%    \caption{Scatter plots of the predicted delays and ground-truth delays}
%    \label{fig:on-off_scatter}
%\end{figure*}
%
%\subsection{Performance Measures}
%In order to evaluate the performance of the delay predictors, we consider two measures: \emph{absolute bias} and \emph{mean squared error} (MSE) for accuracy and precision, respectively. The absolute bias is defined as $\text{Bias}(\widehat{W}) = |E[W - \widehat{W}]|$ and will be approximated by 
%\begin{equation}
%\widehat{\text{Bias}} = \left|\frac{1}{N_{sample}} \sum_{i=1}^{N_{sample}} (d_i-p_i)\right|,
%\end{equation}
%where $d_i$ and $p_i$ are the ground-truth and predicted waiting times for the $i^{th}$ data point. 
%
%The other measure is defined as $\text{MSE}(\widehat{W}) = E[(W-\widehat{W})^2]$ and will be approximated by the \emph{average squared error} as follows:
%
%\begin{equation}
%\text{ASE} = \frac{1}{N_{sample}} \sum_{i=1}^{N_{sample}} (d_i-p_i)^2.
%\end{equation}
%
%\subsection{Simulation Experiments}
%In the rest of this section, we present our results on delay prediction and distribution estimation in multi-server queueing systems. Let us begin with a short description of the arrival and service processes that are used in the following experiments. First, we consider a deterministic ON-OFF arrival process which can be used for simple approximation of a system with batch arrivals, such as transport terminals, in which arrival and departures occur in batches based on schedules. The ON-OFF arrivals have a cycle length of $4$ hours and a duty cycle equal to $75\%$. The second type of time-varying arrivals that are used in the experiments is the Non-homogeneous Poisson process (NHPP), which is a good fit for arrivals in hospitals and call centers~\cite{nhpp}. We adopt the same model as in~\cite{iw2011a} with sinusoidal arrival rate to capture the daily cycles, i.e., we consider an arrival rate of $\lambda(t) = \bar{\lambda}(1+\alpha \sin(2 \pi t/T))$, where  $\bar{\lambda}$, $\alpha$ and $T$ represent the average arrival rate, relative amplitude and the cycle length of the arrival rate. We have evaluated systems with exponential, lognormal and H2 service times, however, the results are only presented for lognormal service times, due to space considerations.  Moreover, we use an MDN implementation which is based on~\cite{mdn_imp} and uses the Keras deep learning library. The training data set consists of around $27000$ samples and the test results are evaluated on $5000$ sample customers. As mentioned earlier, since we are studying delay-history-based predictors, we only consider delay of the last $h$ customers to enter service as the feature set. The simulation parameters are summarized in Table~\ref{ta:sim_table}. 
%
%
%\begin{table}[t!]
%\centering
%\caption{Parameters of the simulation.}
%\begin{tabular}[t]{llr}
%\hline
%%\rowcolor{Gray}
%$\text{Notation}$ & Definition & value\\ 
%\hline
%$E[s]$ & Mean service time & 1 (10 mins)\\ 
%$\rho$ & Traffic intensity & 0.95\\
%$T$ & Cycle of NHPP arrivals & 144 (1 day)\\ 
%$\alpha$ & Relative amplitude of $\lambda(t)$ & 0.5\\ 
%$C$ & Number of servers & 20\\
%%\rowcolor{Gray}
%\end{tabular}\label{ta:sim_table}
%\end{table}
%
%In the first experiment, we consider a multi-server queueing system with $20$ servers, deterministic ON-OFF arrival and lognormal service times. We use a simple feed-forward neural network to approximate the conditional mean of the delay given previous history, i.e., $E[W(\bold{w}_h)]$, and use it as our predictor. Fig.~\ref{fig:on-off_scatter} shows the scatter plots of the ground-truth and predicted delays for the LES predictor, and three other NN-based predictors with delay history lengths of $1, 25$ and $50$. As can be seen in Fig.~\ref{fig:on-off_scatter}.a, there exists a time lag between the LES delays and the ground-truth delays, particularly when the system is busy and the ground-truth values are large. On the other hand, we can observe that even a simple feed-forward neural network which only relies on the LES delay can achieve a much better performance and reduce the MSE by around $65\%$ compared to the LES predictor (see Fig.~\ref{fig:on-off_scatter}.b). Furthermore, the absolute bias has been reduced tremendously, which suggests that the systematic time lag does not exist anymore. It seems that increasing the delay history information does not have a noticeable impact on MSE in this experiment and might even result in overfitting and therefore a larger MSE (Fig.~\ref{fig:on-off_scatter}.d). From Fig.~\ref{fig:on-off_scatter} we can observe that the predictors can have large errors when the ground-truth delay is very small. One explanation might be that large past delays can either imply large delays for the next customers if the ON period continues, or suggest very small delays if the arrival process goes to the OFF state.
%The vertical group of the outliers around zero ground-truth delay represent this phenomenon. 
%
%%because of the rapid transitions of the arrival process from ON to OFF states and vice versa, the predictors might not be able to make good predictions
%
%\begin{figure*}[t!]
%\centering
%\includegraphics[scale=0.38]{nhpp_scatter.png}
%    \caption{Scatter plots of the predicted delays and ground-truth delays}
%    \label{fig:nhpp_scatter}
%\end{figure*}
%
%\begin{figure}[t!]
%\centering
%\includegraphics[scale = 0.5]{pdfs.eps}
%    \caption{Estimated probability density function $P(W|w_1)$, for $w_1 = 5, 10$ and $15$. }
%    \label{fig:pdfs}
%\end{figure}
%
%Now, consider the same queueing system but with NHPP arrivals. Fig.~\ref{fig:nhpp_scatter} shows the scatter plots for the same set of predictors. Similar to Fig.~\ref{fig:on-off_scatter}, there is a time lag between the LES delays and the ground-truth values. Moreover, Fig.~\ref{fig:nhpp_scatter}.a suggests that the conditional distribution of the delay given LES delay information should be multimodal. In other words, a particular LES delay can suggest both larger or smaller future delays, depending on whether the arrival rate and therefore system backlog, is in the increasing or decreasing phase. We observe that by increasing the length of the delay history to $h=50$, the NN-based predictor can better learn whether the system backlog is in the increasing or decreasing phase and hence, it is able to reduce the MSE by around $75\%$.
%
%As we mentioned earlier, single value predictions of the waiting times might not be very informative and we are interested in more descriptive statistics of the system. For instance, it is more desirable to obtain stochastic upper bounds or lower bounds on a customer's delay similar to Eqs.~(\ref{ub_bound}) and (\ref{lb_bound}), rather than providing a single value prediction. In order to achieve this goal, we use MDNs as described in Section~\ref{mdn} to estimate the conditional distribution of the waiting time given delay history of the last $h$ customers to enter service. Fig.~\ref{fig:pdfs} shows the predicted conditional distribution of the waiting time in the previous experiment with NHPP arrivals, given LES delays equal to $5$, $10$ and $15$, i.e., $P(W|\bold{w}_1=5)$, $P(W|\bold{w}_1=10)$ and $P(W|\bold{w}_1=15)$, respectively. The two modes in the estimated distribution function, correspond to the two groups of points in the scatter plot shown in Fig.~\ref{fig:nhpp_scatter}.a, with the same LES delay value. Moreover,  Fig.~\ref{fig:pdfs} suggests that given a particular LES delay, it is more likely to have a larger delay for the new arrival. This can be explained by the fact that most of the customers with the same LES delay should have entered the system in the increasing phase of the arrival rate, while the queue length is growing, and therefore they are more likely to experience larger delays than the LES customer.
%
%
%Now, we use the estimated conditional distributions in a more effective way to obtain probabilistic bounds on the waiting time of a new arrival. Fig.~\ref{fig:bounds} shows a sample path of the waiting times in the previous experiment with NHPP arrivals for a period of two days. The stochastic upper bound and lower bound calculated from Eqs.~(\ref{ub_bound}) and (\ref{lb_bound}) are also shown in Fig.~\ref{fig:bounds}. The stochastic bounds are calculated to hold with a probability more than $0.95$, i.e, $P_{ub}=P_{lb}=0.05$. It should be mentioned that increasing the confidence probability can result in looser bounds. As mentioned earlier, the calculated upper bounds are good candidates for delay announcements. Closely related to these bounds, we can find the confidence intervals for each prediction using Eq.~(\ref{eq:conf_int}) and the predicted distributions. Fig.~\ref{fig:confInterval} shows the same sample path of the waiting times as in Fig.~\ref{fig:bounds}, along with the MMSE predictions and $95\%$ confidence intervals. We should emphasize that the confidence intervals are calculated based on the predicted distributions, rather than a simple Gaussian assumption. It can be observed that the confidence intervals can be pretty large for longer waiting times, which shows the importance of considering other statistics instead of focusing on single value predictions.
%
%\begin{figure}[t!]
%\centering
%\includegraphics[scale=0.33]{bounds.eps}
%    \caption{Probabilistic upper bound and lower bound on the waiting times with less than $5\%$ violation probabilities, given delay history of the last $h=50$ customers who entered service.}
%    \label{fig:bounds}
%\end{figure}
%
%\begin{figure}[t!]
%\centering
%\includegraphics[scale=0.33]{confInterval.eps}
%    \caption{MMSE predictions along with 95\% confidence intervals, given delay history length of $h=50$.}
%    \label{fig:confInterval}
%\end{figure}
%First, let us begin with the case of one-step ahead prediction, where we are interested in predicting the distribution of a new arrival's waiting time given the delay of the LES customer. We consider interarrival times with exponential ($c_U = 1$) and hyperexponential (H2 with $c_S = 2$) distributions. For the service times, we consider exponential and lognormal distributions ($LN(1,4)$). The H2 and $LN(1,4)$ distributions have higher variability compared to the exponential distribution. The learned conditional distributions of the delays are presented in quantile-quantile (Q-Q) plots in Fig.\ref{}, where the quantiles of the learned distribution are compared with those of the simulation in $10\%$ increments. Moreover, the quantiles of the Gaussian approximation from~\cite{} have been included for comparison.  It can be seen that the learned distribution better predicts the tails of the delay distribution compared to a single Gaussian case. This particularly can be helpful in finding more accurate statistical upper or lower bounds on the conditional delay, i.e., $P(W(w_1) > w_{up})<\epsilon$ or $P(W(w_1) < w_{lb})<\epsilon$.
%
%The mean and the variance of the predicted mixture model are shown in Fig.~\ref{}. The predicted values are in close agreement with those of simulation results and theoretical estimates from~\cite{}. It should be noted that the learned model only uses the delay history and has no explicit information about the number of servers or traffic intensity. 
%\subsection{m-step Ahead Predictions}
